Machine Learning-based Selection of Graph Partitioning Strategy Using the Characteristics of Graph Data and Algorithm

Analyzing large graph data is an essential part of many modern applications, such as social networks. Due to its large computational complexity, distributed processing is frequently employed. This requires graph data to be divided across nodes, and the choice of partitioning strategy has a great impact on the execution time of the task. Yet, there is no one-size-fits-all partitioning strategy that performs well on arbitrary graph data and algorithms. The performance of a strategy depends on the characteristics of the graph data and algorithms. Moreover, due to the complexity of graph data and algorithms, manually identifying the best partitioning strategy is also infeasible. In this work, we propose a machine learning-based approach to select the most appropriate partitioning strategy for a given graph and processing algorithm. Our approach enumerates viable partitioning strategies, predicts the execution time of the target algorithm for each, and selects the partitioning strategy with the fastest estimated execution time. Our machine learning model is trained on features extracted from graph data and algorithm pseudo-code. We also propose a method that augments real execution logs of graph tasks to create a large synthetic dataset. Evaluation results show that the strategies selected by our approach lead to 1.46X faster execution time on average compared with the mean execution time of the partitioning strategies and about 0.95X the performance compared to the best partitioning strategy.

==> figure/all_result.tex <==
\begin{figure*}[ht]
\subfloat[Evaluation score on datasets \label{figure:data_result}]{\includegraphics[width=1.9\columnwidth]{image/chosen_image/score_data_all.jpg}}
\vspace{1mm}

\subfloat[Evaluation score on algorithms \label{figure:app_result}]{\includegraphics[width=1.9\columnwidth]{image/chosen_image/score_algo_all.jpg}}

\caption{Evaluation score, X axis: Graph Data/Algorithms, Y axis: Score(best/avg/worst). For visualization, the top 1 point above 10 points were not represented in the $Score_{avg}$ graph, and the top 8 points above 10 points were not represented in the $Score_{worst}$ graph.}
\label{figure:all_result}
\end{figure*}

==> figure/intro_example.tex <==
\begin{figure}[t]
\label{fig 1}
\centering
\begin{subfigure}{0.45\textwidth}
%1\textwidth
%\linewidth
\includegraphics[width=1\textwidth, height=30mm]{Conference-LaTeX-template_7-9-18/image/figure_1_aaaa.png}
\caption{Computation time on different data set} \label{fig:1a}
\end{subfigure}
\newline
%\hspace*{\fill}
\begin{subfigure}{0.45\textwidth}
\includegraphics[width=1\textwidth]{Conference-LaTeX-template_7-9-18/image/figure_1_bbb.png}
\caption{Computation time on different application} \label{fig:1b}
\end{subfigure}
\caption{Computation time on several data sets and applications} \label{fig:1}
\end{figure}


==> figure/intro_example_0826.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.3\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Conference-LaTeX-template_7-9-18/image/fig1/CC_6_basic_test.png}
        \caption[Network2]%
        {{\small \textit{dblp}/\textbf{CC}}}    
        \label{fig:1a}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\columnwidth}  
        \centering 
        \includegraphics[width=\textwidth]{Conference-LaTeX-template_7-9-18/image/fig1/PR_6_basic_test.png}
        \caption[]%
        {{\small \textit{dblp}/\textbf{PR}}}    
        \label{fig:1b}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\columnwidth}   
        \centering 
        \includegraphics[width=\textwidth]{Conference-LaTeX-template_7-9-18/image/fig1/GC_6_basic_test.png}
        \caption[]%
        {{\small \textit{dblp}/\textbf{GC}}}    
        \label{fig:1c}
    \end{subfigure}
    \vskip\baselineskip
    
    
    \begin{subfigure}[b]{0.3\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Conference-LaTeX-template_7-9-18/image/fig1/CC_6_basic_test.png}
        \caption[Network2]%
        {{\small \textit{dblp}/\textbf{CC}}}    
        \label{fig:1d}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\columnwidth}  
        \centering 
        \includegraphics[width=\textwidth]{Conference-LaTeX-template_7-9-18/image/fig1/CC_7_basic_test.png}
        \caption[]%
        {{\small \textit{road\_ca}/\textbf{CC}}}
        \label{fig:1e}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\columnwidth}   
        \centering 
        \includegraphics[width=\textwidth]{Conference-LaTeX-template_7-9-18/image/fig1/CC_11_basic_test.png}
        \caption[]%
        {{\small \textit{stanford}/\textbf{CC}}}
        \label{fig:1f}
    \end{subfigure}
    \caption[ The average and standard deviation of critical parameters ]
    {\small Application performance. Each subfigure represents the application performance of some specific datasets and algorithms. The caption of each figure is the name of the dataset and the algorithm where the application was executed. Details can be found in Table \ref{tab:dataset_table2}and section \ref{app_list}. The PS\_ID at the bottom of each figure means the ID of the partitioning strategies, which is depicted in Table \ref{table:partition_strategies}. In (a), (b), and (c), the application performance for the same dataset, and different algorithms is depicted, the relative performance is different depending on the algorithm. (d), (e), and (f) shows the performance for the same algorithm and different datasets. Relative performance is different, as in (a), (b), and (c). This implies it is important to select a partitioning strategy by comprehending the algorithm's features and data from this result.} 
    \label{fig:1}
\end{figure}


% Engine scalability test on the \emph{Web-Stanford} graphs with \emph{Ginger} partitioning strategy and increasing machines.











% \begin{figure}
% \centering
% \begin{subsubcaption}
% \label{1--a}
% \begin{subfigure}{2.9cm}
% \includegraphics[width=\linewidth]{Conference-LaTeX-template_7-9-18/image/fig1/CC_6_basic_test.png}
% \caption{DID: 6, AID: 5}\label{1--a--1} % DID: 6, AID: 10
% \end{subfigure}%\qquad
% \begin{subfigure}{2.9cm}
% \includegraphics[width=\linewidth]{Conference-LaTeX-template_7-9-18/image/fig1/GC_6_basic_test.png}
% \caption{DID:6, AID:3}\label{1--a--2}
% \end{subfigure}%\qquad
% \begin{subfigure}{2.9cm}
% \includegraphics[width=\linewidth]{Conference-LaTeX-template_7-9-18/image/fig1/PR_6_basic_test.png}
% \caption{DID:6, AID:2}\label{1--a--3}
% \end{subfigure}
% \end{subsubcaption}

% \begin{subsubcaption}
% \label{1--b}
% \begin{subfigure}{2.9cm}
% \includegraphics[width=\linewidth]{Conference-LaTeX-template_7-9-18/image/fig1/CC_6_basic_test.png}
% \caption{DID:6, AID:5}\label{1--b--1}
% \end{subfigure} %\hspace{0.2cm}%\qquad
% \begin{subfigure}{2.9cm}
% \includegraphics[width=\linewidth]{Conference-LaTeX-template_7-9-18/image/fig1/CC_7_basic_test.png}
% \caption{DID:7, AID:5}\label{1--b--2}
% \end{subfigure}%\qquad
% \begin{subfigure}{2.9cm}
% \includegraphics[width=\linewidth]{Conference-LaTeX-template_7-9-18/image/fig1/CC_11_basic_test.png}
% \caption{DID:11, AID:5}\label{1--b--3}
% \end{subfigure}
% \end{subsubcaption}

% \caption{Application performance. Each subfigure represents the application performance of all partitioning strategies covered in this paper for a specific dataset and algorithm. DID implies for graph dataset ID, AID implies for algorithm ID, and PSID implies for partitioning strategy ID, which can be found in Table \ref{tab:dataset_table2}, section \ref{app_list}, and Table \ref{table:partition_strategies}. In (a), the application performance for the same dataset, and different algorithms is depicted, the relative performance is different depending on the algorithm. (b) shows the performance for the same algorithm and different datasets. Relative performance is different, as in (a). We believe it is important to select a partitioning strategy by comprehending the algorithm's features and data from this result.}
% % 어플리케이션 퍼포먼스, 각 sugfigure는 특정 dataset과 algorithm에 대해 본 페이퍼에서 다루는 모든 partitioning strategy의 application performance를 나타냅니다. DID는 graph dataset ID를, AID는 algorithm ID를 의미하며 이는 Table \ref{tab:dataset_table2}과 section \ref{app_list}에서 확인할 수 있습니다. (a)에서는 같은 dataset, 각기 다른 algorithm에 대한 application performance를 나타내는데, algorithm에 따라 상대적인 퍼포먼스가 다른 것을 확인할 수 있습니다. (b)에서는 같은 algorithm, 각기 다른 dataset에 대한 performace를 나타냅니다. (a)와 마찬가지의 결과를 확인할 수 있습니다. 우리는 이 결과에서 algorithm과 data에 대한 feature를 파악하여 partitioning strategy를 선택하는 것이 중요하다고 여깁니다.
% \end{figure}

% %References:
% %\ref{a--1} and \subref{a--1};
% %\ref{b--1} and \subref{b--1}.

==> figure/mapping_ex.tex <==
\begin{figure}[ht]
\begin{center}
  \includegraphics[width=1\columnwidth]{Conference-LaTeX-template_7-9-18/image/mapping_ex.png}
  \caption{Vertex Mapping Example. This figure shows the vertex-worker mapping formed for the of the example graph partition in Fig \ref{fig:distributed_graph}.}
  \label{fig:mapping_ex}
\end{center}
\vspace{-0.5cm}
\end{figure}

==> figure/overall.tex <==
\begin{figure}[t]
\begin{center}
  \includegraphics[width=0.9\columnwidth]{Conference-LaTeX-template_7-9-18/image/Overall_v3.png}
  \caption{Overall structure of ETRM.}
  \label{fig:overall}
\end{center}
\vspace{-0.5cm}
\end{figure}

==> figure/pagerank_code.tex <==
\begin{figure}[h]
\begin{center}
  \includegraphics[width=0.9\columnwidth]{Conference-LaTeX-template_7-9-18/image/pagerank.png}
  \caption{Code analysis on PageRank algorithm}
  \label{fig:PR-analysis}
\end{center}
\end{figure}

==> figure/r2.tex <==
\begin{figure}[]
\begin{center}
  \includegraphics[width=1\columnwidth, height=35mm]{Conference-LaTeX-template_7-9-18/image/r2.png}
  \caption{Real VS Predicted computation time on composed data}
  \label{fig:r2}
\end{center}
\end{figure}

==> figure/real_pred.tex <==
\begin{figure}[]
\centering
\subfloat[Real, DID: 2, AID: 10 \label{p1}]{\includegraphics[width=0.45\columnwidth, height=30mm]{Conference-LaTeX-template_7-9-18/image/DID_2_Algo_Clustering Coefficient_Real.png}} 
\hspace{0.1cm}
\subfloat[Pred, DID: 2, AID: 10 \label{p2}]{\includegraphics[width=0.45\columnwidth, height=30mm]{Conference-LaTeX-template_7-9-18/image/DID_2_Algo_Clustering Coefficient_Pred.png}} 
\vspace{1mm}

\subfloat[Real, DID: 4, AID: 0 \label{p3}]{\includegraphics[width=0.45\columnwidth, height=30mm]{Conference-LaTeX-template_7-9-18/image/DID_4_Algo_Get Out-Degree_Real.png}} 
\hspace{0.1cm}
\subfloat[Pred, DID: 4, AID: 0 \label{p4}]{\includegraphics[width=0.45\columnwidth, height=30mm]{Conference-LaTeX-template_7-9-18/image/DID_4_Algo_Get Out-Degree_Pred.png}} 
\vspace{1mm}

\subfloat[Real, DID: 7, AID: 5 \label{p5}]{\includegraphics[width=0.45\columnwidth, height=30mm]{Conference-LaTeX-template_7-9-18/image/DID_7_Algo_SSSP_Real.png}} 
\hspace{0.1cm}
\subfloat[Pred, DID: 7, AID: 5 \label{p6}]{\includegraphics[width=0.45\columnwidth, height=30mm]{Conference-LaTeX-template_7-9-18/image/DID_7_Algo_SSSP_Pred.png}} 

\caption{Real/Predicted computation time on test records, X axis: Partitioning Strategy ID, Y axis: computation time. Green indicates the recommended partitioning strategy and best strategy match, red means the actual best strategy, gray means the recommended partitioning strategy, and blue and orange respectively indicates the actual/predicted computation time.}
\label{real/pred}
\end{figure}



%\begin{center}
%  \includegraphics[width=1\columnwidth, height=40mm]{Conference-LaTeX-template_7-9-18/image/r2.png}
%  \caption{Real VS Prediction}
%  \label{fig:r2}
%\end{center}
%\vspace{-0.5cm}

==> figure/recscore.tex <==
\begin{figure}[h]
\begin{center}
  \includegraphics[width=1\columnwidth, height=40mm]{Conference-LaTeX-template_7-9-18/image/RecScore.png}
  \caption{RecScore}
  \label{fig:recscore}
\end{center}
\end{figure}

==> figure/syn.tex <==
\begin{figure}[t]
\begin{center}
  \includegraphics[width=0.9\columnwidth]{Conference-LaTeX-template_7-9-18/image/synthetic8.png}
  \caption{Combinated Training Dataset}
  \label{fig:syn_train_data}
\end{center}
\vspace{-0.5cm}
\end{figure}

==> figure/temp.tex <==
\begin{figure*}[t]
\begin{center}
  \includegraphics[width=2\columnwidth]{Conference-LaTeX-template_7-9-18/image/mape.png}
  \caption{MAPE matrix.}
  \label{fig:mape}
\end{center}
\vspace{-0.5cm}
\end{figure*}

==> table/dataset.tex <==
\begin{table}[]
\caption{}
\label{tab:dataset_table}
\begin{tabular}{|c|c|c|c|c|}
\hline
Data set         & Nodes   & Edges   & Direction  & Description                           \\ \hline
ego-Facebook     & 4039    & 88234   & Undirected & Social circles from Facebook          \\ \hline
wiki-Vote        & 7115    & 103689  & Directed   & Wikipedia   who-votes-on-whom network \\ \hline
gemsec-Deezer-RO & 41773   & 125826  & Undirected & Gemsec Deezer dataset                 \\ \hline
gemsec-Deezer-HU & 47538   & 222887  & Undirected & Gemsec Deezer dataset                 \\ \hline
gemsec-Deezer-HR & 54573   & 498202  & Undirected & Gemsec Deezer dataset                 \\ \hline
soc-Epinions1           & 75879  & 508837  & Directed & Who-trusts-whom   network of Epinions.com                 \\ \hline
soc-sign-Slashdot081106 & 77350  & 516575  & Directed & Slashdot Zoo signed   social network from November 6 2008 \\ \hline
amazon0302              & 262111 & 1234877 & Directed & Amazon product   co-purchasing network from March 2 2003  \\ \hline
web-Stanford     & 281903  & 2312497 & Directed   & Web graph of   Stanford.edu           \\ \hline
com-DBLP         & 317080  & 1049866 & Undirected & DBLP collaboration network            \\ \hline
com-Amazon       & 334863  & 925872  & Undirected & Amazon product network                \\ \hline
roadNet-CA       & 1965206 & 2766607 & Undirected & Road network of California            \\ \hline
\end{tabular}
\end{table}

==> table/mape.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[t]
\caption{MAPE result}
\label{table:mape}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccccccc}
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{\textbf{MAPE}}} & \multicolumn{6}{c}{Test set D, B} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}avg on \\ graph data D, B\end{tabular}} & \multicolumn{2}{c}{Test set C, A} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}avg on \\ graph data C, A\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}avg on \\ graph data\end{tabular}} \\
\multicolumn{2}{c}{} & \textbf{AID} & \textbf{AOD} & \textbf{PR} & \textbf{GC} & \textbf{APCN} & \textbf{TC} &  & \textbf{CC} & \textbf{RW} &  &  \\
\midrule
\multirow{8}{*}{Test set D, C} & \textit{facebook} & 1.4729 & 0.6524 & 0.0999 & 0.1304 & 0.0861 & 0.3832 & 0.4708 & 0.8817 & 0.8452 & 0.8635 & 0.5690 \\
 & \textit{wiki} & 1.7054 & 0.8951 & 0.1489 & 0.1840 & 0.0954 & 0.1408 & 0.5283 & 0.5940 & 1.2265 & 0.9103 & 0.6238 \\
 & \textit{epinions} & 1.9871 & 1.2959 & 0.1812 & 0.0349 & 0.0854 & 0.2477 & 0.6387 & 0.8705 & 3.6400 & 2.2553 & 1.0429 \\
 & \textit{amazon-1} & 1.6562 & 1.2355 & 0.1214 & 0.0298 & 0.2996 & 0.4613 & 0.6340 & 0.7111 & 1.9715 & 1.3413 & 0.8108 \\
 & \textit{slashdot} & 0.7047 & 0.4147 & 0.1194 & 0.1094 & 0.0694 & 0.2222 & 0.2733 & 0.5994 & 1.7382 & 1.1688 & 0.4972 \\
 & \textit{amazon-2} & 0.1860 & 0.1116 & 0.1373 & 0.0498 & 0.7589 & 0.3816 & 0.2709 & 0.5675 & 0.4498 & 0.5086 & 0.3303 \\
 & \textit{dblp} & 0.2433 & 0.2094 & 0.0880 & 0.0281 & 0.6457 & 0.3110 & 0.2543 & 0.4875 & 0.3598 & 0.4237 & 0.2966 \\
 & \textit{road-ca} & 0.5052 & 0.2789 & 0.1427 & 0.1209 & 1.0088 & 0.2156 & 0.3787 & 0.4113 & 0.9889 & 0.7001 & 0.4590 \\
  \hdashline
\multicolumn{2}{c}{avg on algorithm D, C} & 1.0576 & 0.6367 & 0.1298 & 0.0859 & 0.3812 & 0.2954 & 0.4311 & 0.6404 & 1.4025 & 1.0214 & 0.5787 \\
 \hdashline
\multirow{4}{*}{Test set B, A} & \textit{gd-ro} & 1.5453 & 1.6929 & 1.0567 & 0.2972 & 55.0243 & 1.0105 & 10.1045 & 1.4333 & 1.9505 & 1.6919 & 8.0013 \\
 & \textit{gd-hu} & 0.2154 & 0.4232 & 0.3798 & 0.0548 & 32.9838 & 0.3299 & 5.7311 & 0.6205 & 0.8399 & 0.7302 & 4.4809 \\
 & \textit{gd-hr} & 0.1045 & 0.1082 & 0.1106 & 0.2130 & 11.4609 & 0.1441 & 2.0235 & 0.2920 & 0.2707 & 0.2814 & 1.5880 \\
 & \textit{stanford} & 0.1911 & 0.1626 & 0.1670 & 0.0625 & 0.9789 & 0.8542 & 0.4027 & 0.7099 & 0.1929 & 0.4514 & 0.4149 \\
  \hdashline
\multicolumn{2}{c}{avg on algorithm B, A} & 0.5141 & 0.5967 & 0.4285 & 0.1569 & 25.1120 & 0.5847 & 4.5655 & 0.7639 & 0.8135 & 0.7887 & 3.6213 \\
 \hdashline
\multicolumn{2}{c}{avg on algorithm} & 0.8764 & 0.6234 & 0.2294 & 0.1096 & 8.6248 & 0.3919 & 1.8092 & 0.6816 & 1.2062 & 0.9439 & 1.5929 \\
\bottomrule
\end{tabular}%
}
\end{table*}



% \begin{tabular}{ccrrrrrrrrrrrrrr}
% \toprule
% \multicolumn{2}{c}{\multirow{2}{*}{MAPE}} & \multicolumn{6}{c}{Trained Algorithms (A)} & \multicolumn{1}{c}{\multirow{2}{*}{avg\_trained}} & \multicolumn{5}{c}{Unseen Algorithms (B)} & \multicolumn{1}{c}{\multirow{2}{*}{avg\_unseen}} & \multicolumn{1}{c}{\multirow{2}{*}{average}} \\ 
% \multicolumn{2}{c}{} & \multicolumn{1}{c}{\textbf{AID}} & \multicolumn{1}{c}{\textbf{AOD}} & \multicolumn{1}{c}{\textbf{PR}} & \multicolumn{1}{c}{\textbf{GC}} & \multicolumn{1}{c}{\textbf{RW}} & \multicolumn{1}{c}{\textbf{CC}} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{TC}} & \multicolumn{1}{c}{\textbf{CN}} & \multicolumn{1}{c}{\textbf{BFSI}} & \multicolumn{1}{c}{\textbf{BFSO}} & \multicolumn{1}{c}{\textbf{SSSP}} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\ 
% \midrule
% \multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Trained\\ Datasets\\ (1)\end{tabular}} & \textit{facebook} & 0.752 & 1.024 & 0.087 & 0.104 & 0.088 & 0.064 & 0.353 & 0.890 & 1942.330 & 105.399 & 79.605 & 0.669 & 532.001 & 193.729 \\  
%  & \textit{wikivote} & 5.412 & 3.077 & 0.071 & 0.283 & 0.131 & 0.039 & 1.502 & 0.500 & 3784.350 & 757.140 & 132.980 & 996.285 & 1417.689 & 516.388 \\  
%  & \textit{epinions} & 0.682 & 0.495 & 0.079 & 0.174 & 0.030 & 0.085 & 0.257 & 0.960 & 290.198 & 27.741 & 33.790 & 0.908 & 88.159 & 32.286 \\  
%  & \textit{amazon-1} & 0.375 & 0.251 & 0.034 & 0.211 & 0.081 & 0.256 & 0.201 & 0.919 & 2536.670 & 799.759 & 38.367 & 0.643 & 843.860 & 307.052 \\  
%  & \textit{slashdot} & 0.357 & 0.284 & 0.114 & 0.250 & 0.131 & 0.036 & 0.195 & 0.979 & 318.287 & 5.920 & 4.904 & 0.982 & 82.523 & 30.204 \\  
%  & \textit{amazon-2} & 0.226 & 0.199 & 0.076 & 0.140 & 0.046 & 0.049 & 0.122 & 0.890 & 1467.500 & 103.623 & 79.085 & 625.746 & 568.989 & 207.053 \\  
%  & \textit{dblp} & 0.299 & 0.289 & 0.080 & 0.160 & 0.095 & 0.053 & 0.163 & 0.891 & 1124.620 & 41.186 & 64.411 & 0.251 & 307.617 & 112.030 \\  
%  & \textit{road\_ca} & 0.239 & 0.190 & 0.071 & 0.020 & 0.132 & 0.054 & 0.118 & 8.362 & 5609.900 & 280543 & 271620 & 0.995 & 139443.474 & 50707.600 \\ 
%  \hdashline
% \multicolumn{2}{c}{avg\_trained} & 1.043 & 0.726 & 0.077 & 0.168 & 0.092 & 0.079 & 0.364 & 1.799 & 2134.232 & 35297.971 & 34006 & 203.310 & 14328.791 & 7164.434 \\ 
% \hdashline
% \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Unseen\\ Datasets\\ (2)\end{tabular}} & \textit{gd-ro} & 6.657 & 5.660 & 7.811 & 3.294 & 6.482 & 10.762 & 6.778 & 5.275 & 2540.530 & 565.791 & 499.503 & 2.460 & 902.071 & 332.202 \\  
%  & \textit{gd-hu} & 3.419 & 2.988 & 3.226 & 1.419 & 3.208 & 5.414 & 3.279 & 0.494 & 2186.630 & 144.875 & 133.771 & 0.167 & 616.361 & 225.965 \\  
%  & \textit{gd-hr} & 0.800 & 0.811 & 0.457 & 1.550 & 1.299 & 0.892 & 0.968 & 0.849 & 1619.220 & 58.717 & 80.416 & 0.414 & 439.692 & 160.493 \\  
%  & \textit{stanford} & 0.343 & 0.365 & 0.168 & 0.155 & 0.685 & 0.933 & 0.442 & 0.964 & 2778.540 & 549.529 & 1137.050 & 294.904 & 1190.006 & 433.058 \\ 
%  \hdashline
% \multicolumn{2}{c}{avg\_unseen} & 2.805 & 2.456 & 2.916 & 1.604 & 2.919 & 4.500 & 2.867 & 1.896 & 2281.230 & 329.728 & 462.685 & 74.486 & 630.005 & 287.929 \\ 
% \hdashline
% \multicolumn{2}{c}{average} & 1.630 & 1.303 & 1.023 & 0.647 & 1.034 & 1.553 & 1.198 & 1.831 & 2183.230 & 23641.900 & 22825.300 & 160.369 & 9762.529 & 4438.170 \\ 
% \bottomrule
% \end{tabular}%
% }
% \end{table*}

==> table/motivation.tex <==
\begin{table}[]
\centering
\caption{Motivation Example}
\label{tab:motivation}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\begin{tabular}[c]{@{}c@{}}Task\\ ID\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Graph\\ Data\end{tabular} &
  Algorithm &
  \begin{tabular}[c]{@{}c@{}}Best\\ Partitioning\\ Strategy\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Fastest \\ Execution\\ Time\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Worst\\ Partitioning\\ Strategy\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Slowest\\ Execution\\ Time\end{tabular} \\ \hline
1 &
  Epinions &
  PageRank &
  HDRF-50 &
  1.61 &
  \begin{tabular}[c]{@{}c@{}}Random\\ (GraphX)\end{tabular} &
  4.10 \\ \hline
2 &
  2 &
  \begin{tabular}[c]{@{}c@{}}Single Source \\ Shortest Path\end{tabular} &
  2 &
  22.70 &
  0 &
  163.50 \\ \hline
3 &
  DBLP &
  PageRank &
  HDRF-10 &
  6.63 &
  \begin{tabular}[c]{@{}c@{}}2D-Edge \\ Partition\end{tabular} &
  14.30 \\ \hline
4 &
  DBLP &
  \begin{tabular}[c]{@{}c@{}}Clustering\\ Coefficient\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}2D-Edge\\ Partition\end{tabular} &
  94.36 &
  HDRF-50 &
  273.48 \\ \hline
5 &
  DBLP &
  GraphColoring &
  HDRF-10 &
  20.67 &
  \begin{tabular}[c]{@{}c@{}}2D-Edge\\ Partition\end{tabular} &
  26.57 \\ \hline
6 &
  Amazon &
  PageRank &
  0 &
  8.89 &
  10 &
  30.91 \\ \hline
7 &
  Amazon &
  GraphColoring &
  11 &
  21.25 &
  10 &
  63.09 \\ \hline
8 &
  \begin{tabular}[c]{@{}c@{}}Gemsec\\ Deezer-RO\end{tabular} &
  PageRank &
  0 &
  1.03 &
  9 &
  2.74 \\ \hline
9 &
  7 &
  \begin{tabular}[c]{@{}c@{}}Clustering\\ Coefficient\end{tabular} &
  3 &
  197.21 &
  2 &
  235.747 \\ \hline
\end{tabular}
\end{table}

==> table/motivation2.tex <==
\begin{table}[]
\centering
\caption{Motivating Example. The best and worst partitioning strategy is different for each workload.}
\label{tab:motivation}
\begin{tabular}{ccccc}
\hline
\begin{tabular}[c]{@{}c@{}}\textbf{Task}\\ \textbf{ID}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\textbf{Graph}\\ \textbf{Data}\end{tabular} &
  \textbf{Algorithm} &
  \begin{tabular}[c]{@{}c@{}}\textbf{Best}\\ \textbf{Partitioning}\\ \textbf{Strategy}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\textbf{Worst}\\ \textbf{Partitioning}\\ \textbf{Strategy}\end{tabular} \\ \hline \hline
\multicolumn{1}{|c|}{1} &
  \multicolumn{1}{c|}{Epinions} &
  \multicolumn{1}{c|}{PageRank} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}HDRF\\ 50\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Random\\ (GraphX)\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{2} &
  \multicolumn{1}{c|}{DBLP} &
  \multicolumn{1}{c|}{PageRank} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}HDRF\\ 10\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}2D-Edge \\ Partition\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{3} &
  \multicolumn{1}{c|}{DBLP} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Clustering\\ Coefficient\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}2D-Edge\\ Partition\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}HDRF\\ 50\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{4} &
  \multicolumn{1}{c|}{DBLP} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Random\\ Walk\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Random\\ (GraphX)\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}2D-Edge \\ Partition\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{5} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}RoadNet\\ CA\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Random\\ Walk\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}HDRF\\ 20\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Random\\ (GraphX)\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{6} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}RoadNet\\ CA\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Clustering\\ Coefficient\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Canonical\\ Random\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Random\\ (GraphX)\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{7} &
  \multicolumn{1}{c|}{Amazon} &
  \multicolumn{1}{c|}{PageRank} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}1D-Edge \\ Partition\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}HDRF\\ 100\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{8} &
  \multicolumn{1}{c|}{Amazon} &
  \multicolumn{1}{c|}{GraphColoring} &
  \multicolumn{1}{c|}{Ginger} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}HDRF\\ 100\end{tabular}} \\ \hline
\end{tabular}
\end{table}
